Towards a Robust Aerial Cinematography Platform: Localizing and Tracking Moving Targets in Unstructured Environments

The use of drones for aerial cinematography has revolutionized several applications and industries that require live and dynamic camera viewpoints such as entertainment, sports, and security. However, safely controlling a drone while filming a moving target usually requires multiple expert human operators; hence the need for an autonomous cinematographer. Current approaches have severe real-life limitations such as requiring fully scripted scenes, high-precision motion-capture systems or GPS tags to localize targets, and prior maps of the environment to avoid obstacles and plan for occlusion. In this work, we overcome such limitations and propose a complete system for aerial cinematography that combines: (1) a vision-based algorithm for target localization; (2) a real-time incremental 3D signed-distance map algorithm for occlusion and safety computation; and (3) a real-time camera motion planner that optimizes smoothness, collisions, occlusions and artistic guidelines. We evaluate robustness and real-time performance in series of field experiments and simulations by tracking dynamic targets moving through unknown, unstructured environments. Finally, we verify that despite removing previous limitations, our system achieves state-of-the-art performance. Videos of the system in action can be seen at https://youtu.be/ZE9MnCVmumc

==> inputs/5_stats.tex <==
% !TEX root = ../root.tex

\subsection{System statistics}
\label{subsec:experiments_stats}

% \rbnote{show useful statistics about system performance that allows us to get useful insights into bottlenecks and give others an idea of what needs improvement in the future}

\chnote{incorporate time takes for one laser scan update, maybe a time statistic table?}
% \rbnote{include stats on: flight time, planning freq, plan time horizon, num iterations max, how much \% of CPU, GPU and RAM each sub-system is taking, time that it takes to update one laser scan}
% \begin{table}[]
%     \caption{Planning parameters used in experiments \chnote{RB: pls confirm values}}
%     \begin{tabular}{l|l}
%     \hline
%     \textbf{Parameter} & \textbf{Value} \\ \hline
%     Planning Freq. & 5 Hz \\
%     Max. Iteration & 100? \\
%     Planning time horizon & 5s \\ \hline
%     \end{tabular}
%     \label{table:planning_param}
% \end{table}
\begin{table}[ht]
        \caption{Planning parameters used in experiments \chnote{step size}}

    \begin{tabular}{llll}
    \hline
    \textbf{Parameter} & Planning Freq. & Max. Iteration & Planning time horizon \\ \hline
    \textbf{Value} & \multicolumn{1}{c}{5Hz} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{10s} \\ \hline
    \end{tabular}
    \label{tab:planning_param}
\end{table}

\begin{table}[ht]
    \caption{Compute Statistics \chnote{add footnotes about detect/track, heading only when tracking}}
    \begin{tabular}{cc|ccc}
        \hline
        \textbf{Subsystem} & \textbf{Module} & \textbf{\% Thread} & \textbf{\% GPU} & \textbf{\% RAM} \\ \hline
        Vision & \begin{tabular}[c]{@{}c@{}}Detection/Tracking\\ Gimbal Control\\ Heading Est.\\ KF\end{tabular} & \begin{tabular}[c]{@{}c@{}}56.6/24.2\\ 9.9\\ 23.5\\ 8.2\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}27.0/0.3\\ 0.6\\ 22.3\\ 1.0\end{tabular} \\ \hline
        Mapping & \begin{tabular}[c]{@{}c@{}}Dist. TF Map\\ Occupancy Map\\ LiDAR Driver\end{tabular} & \begin{tabular}[c]{@{}c@{}}91.0\\ 22.3\\ 23.5\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}9.5\\ 0.6\\ 0.1\end{tabular} \\ \hline
        Planning & CHOMP & 98.3 &  & 9.5 \\ \hline
        Hardware & DJI SDK & 89.7 &  & 0.5
        \end{tabular}
    
\end{table}

\rbnote{add runtime for each module as well? how long it takes (ms) for each part to complete a cycle}

\missingfigure[figwidth=0.5\textwidth]{Time needed for Distance Transform Update over Flight Time. Time decreases as less cells will be updated.}

% \rbnote{maybe say a few tricks I had to do when switching from offline to online map? such as had to significantly decrease threshold for signed distance calculation from 10m to 4m to make computation feasible, and had to significantly lower num of iterations for planner and increase step size to get to solutions much faster and keep re-planning at 5Hz}


==> inputs/6_discussion.tex <==
% !TEX root = ../root.tex

\section{Discussion}
\label{sec:discussion}

% \rbnote{discuss the interesting things that we noticed when going from offline - online map. in terms of computation (much higher CPU load bc of signed distance), changes in planner parameters}

% \rbnote{discuss what hapenned when switched to vision detection versus ground truth GPS: now we are more sentitive in terms of loosing the actor if we do very drastic non smooth motions, plus we must have only the desired actor on camera because it will choose the bounding box where it has higher confidence}

\rbnote{discuss future steps and how we could make system more robust: different strategies for online map to use less CPU, chanigng cost functions to handle multiple actors (artistic cost specifically would change and occlusion a bit), discuss that other types of sensors could be used for different applications like stereo camera pairs to build the evidence grid, and multi-drone scenario}

% \rbnote{maybe talk about future work on shot selection and planner initialization as well?}

